CARMI: A Cache-Aware Learned Index with a Cost-based Construction Algorithm

Learned indexes, which use machine learning models to replace traditional index structures, have shown promising results in recent studies. However, existing learned indexes exhibit a performance gap between synthetic and real-world datasets, making them far from practical indexes. In this paper, we identify that ignoring the importance of data partitioning during model training is the main reason for this problem. Thus, we explicitly apply data partitioning to index construction and propose a new efficient and updatable cache-aware RMI framework, called CARMI. Specifically, we introduce entropy as a metric to quantify and characterize the effectiveness of data partitioning of tree nodes in learned indexes and propose a novel cost model, laying a new theoretical foundation for future research. Then, based on our novel cost model, CARMI can automatically determine tree structures and model types under various datasets and workloads by a hybrid construction algorithm without any manual tuning. Furthermore, since memory accesses limit the performance of RMIs, a new cache-aware design is also applied in CARMI, which makes full use of the characteristics of the CPU cache to effectively reduce the number of memory accesses. Our experimental study shows that CARMI performs better than baselines, achieving an average of 2.2x/1.9x speedup compared to B+ Tree/ALEX, while using only about 0.77x memory space of B+ Tree. On the SOSD platform, CARMI outperforms all baselines, with an average speedup of 1.2x over the nearest competitor RMI, which has been carefully tuned for each dataset in advance.

==> tex/__latexindent_temp.tex <==
\section{Experiments}\label{sec:experiment}



In this section, we conduct experiments to evaluate our cache-aware learned index design and cost-based construction algorithm, and also study several other aspects of CARMI.
\begin{itemize}[leftmargin=5mm]
  \item Section~\ref{sec:setup} lists the basic experimental settings.
  \item Section~\ref{sec:general} shows the general performance of CARMI.
  \item Section~\ref{sec:sosd} reports the results on the SOSD benchmark~\cite{marcus2020benchmarking}.
  \item Section~\ref{sec:tradeoff} demonstrates the possibility of using our cost-based construction algorithm to obtain a fine-grained tradeoff between time and space.
  \item Section~\ref{sec:cost} shows the running time of the index construction algorithm.
  % \item Section~\ref{sec:platform} shows the results of comparative experiments on multiple platforms.
  \techreport{\item \purple{Section~\ref{sec:fanout} demonstrates the effect of the root fanout.}}
  \techreport{\item \purple{Section~\ref{sec:ablation} provides the results of ablation experiments.}}
  \item \paper{A close examination of the index structure details and the ablation experiments can be found in the full technical report~\cite{zhang2021carmi}.} \techreport{\blue{Section~\ref{sec:tree} provides a close examination of several index structures constructed in our experiments.}}
\end{itemize}
\paper{
  \begin{figure*}[ht]
  \centering
  % \setlength{\abovecaptionskip}{-3pt}
  \vspace{-0.6cm}
  \includegraphics[width=0.98\linewidth]{./figure/resultpaper.pdf}
  \vspace{-0.3cm}
  \caption{CARMI vs. Baselines: Time and Space Usage Comparison.}
  \Description{CARMI vs. Baselines: Time and Space Usage Comparison.}
  \label{fig:totalResPaper}
  \vspace{-0.3cm}
\end{figure*}
}

\subsection{Experimental Setup}\label{sec:setup}
We conducted all the single-threaded experiments on an Ubuntu Linux machine equipped with an AMD Ryzen 3700X 8-Core Processor and 32GB RAM.

\subsubsection{Datasets}
Six datasets are used in our main experiments. Their details are listed as follows:
\begin{itemize}[leftmargin=5mm]
  % \item \textbf{longitude dataset:} This dataset is generated from a public dataset of Open Street Maps~\cite{OpenStreetMap}, which includes the latitude and longitude of points around the world. This dataset uses the longitude of points as key, and the number of data points in this dataset is 67,108,864 (the size of each dataset is 1GB). 
  % \item \textbf{longlat dataset:} This dataset is mostly the same as the longitude dataset, except that the key value is computed by: $key=longitude*180+longlat$ as in~\cite{ding2019alex}.
  \item \textbf{OSMC dataset:} This dataset is generated from a public dataset of Open Street Maps~\cite{OpenStreetMap}, which includes the latitude and longitude of points around the world. The number of data points in this dataset is 67,108,864 (the size of each dataset is 1GB).  This dataset is stored as key-value pairs of <$uint64, uint64$>.
  \item \textbf{synthetic dataset:} $4$ synthetic datasets are generated from $4$ different distributions: (a) \textbf{lognormal}: $log(key) \sim \mathcal{N}(0, 1)$; (b) \textbf{uniform}: $key \sim \mathcal{U}(0, 1)$; (c) \textbf{normal}: $key \sim \mathcal{N}(0, 1)$; (d) \textbf{exponential}: $key \sim \text{Exp}(0.25)$. All these datasets are stored as key-value pairs of <$double, double$>. The size of each dataset is 1GB, and the key values of data points are multipled by $10^8$.
  \item \textbf{YCSB dataset}: This dataset consists of 67,108,864 data records generated by YCSB benchmark~\cite{cooper2010benchmarking}. We build an index on the $YCSB\_KEY$ attribute, which obeys a uniform distribution.
\end{itemize}

We have also ported CARMI into the SOSD\techreport{~\cite{marcus2020benchmarking}}\paper{~\cite{sosd-vldb}} platform to test its performance and the details are shown in Section~\ref{sec:sosd}.
  
\techreport{
  \begin{figure*}[t]
    \centering
    % \setlength{\abovecaptionskip}{-3pt}
    \vspace{-0.6cm}
    \includegraphics[width=\linewidth]{./figure/cdf.pdf}
    \caption{The CDFs of Datasets in SOSD~\cite{marcus2020benchmarking}.}
    \Description{The CDFs of Datasets in SOSD~\cite{marcus2020benchmarking}.}
    \label{fig:cdf}
    \vspace{-0.3cm}
  \end{figure*}
}

 \subsubsection{Evaluation Workloads}\label{sec:workload}
  We use 5 different query workloads in our experiments. The first three workloads are similar to the workloads in the YCSB benchmark~\cite{cooper2010benchmarking}: (a) a write-heavy workload with a mix of 50\% reads and 50\% inserts; (b) a read-heavy workload with a mix of 95\% reads and 5\% inserts; (c) a read-only workload. In addition, we include a write-partial workload in which insert operations are concentrated in a small key value range. \techreport{\blue{This workload consists of 85\% reads and 15\% inserts, and the inserted data points are concentrated between 60\% and 90\% of the sorted dataset. The write-partial workload is intended to mimic some real-world scenarios in which the keys of new data points are contained in a small value range during each session (e.g., when using the current date/time as key value).}} Finally, we include a range scan workload with a mix of 95\% range scan and 5\% inserts as in~\cite{ding2019alex}.

 \techreport{
   \blue{For each workload, we evaluate the total time of 100,000 queries (mix of read/write queries), and calculate the average time used by each query. We consider two access patterns for generating the key value of queries: a Zipfian distribution (with parameter 0.99 as in~\cite{ding2019alex}) and a uniform distribution. In workloads involving insert operations, read and insert operations are performed alternately in proportion. For example, in read-heavy workloads, we first perform 19 reads and then perform 1 insert operation. For range scan workloads, the length of each range scan is uniformly sampled from [1, 100].}

  \blue{For the YCSB dataset, the queries are handled differently to simulate real-world use cases: read queries are generated from a Zipfian distribution as usual, but insert key values are sequentially increasing to be consistent with the YCSB benchmark. }
}

\subsubsection{Implementation and Baseline}

We compare against the following baselines: STX B-Tree~\cite{STXBtree} and ALEX~\cite{ding2019alex}. CARMI is open-sourced and can be found on Github~\cite{carmiGithub}. \paper{The default values of parameters in CARMI can be found in our technical report~\cite{zhang2021carmi}.} \techreport{\blue{The default values of parameters in CARMI can be found in the appendix.}} The SOSD benchmark~\cite{marcus2020benchmarking} also includes some read-only learned indexes as baselines in Section~\ref{sec:sosd}.

\subsubsection{Training Queries for Index Construction in CARMI}

In our experiments, the training query workload for index construction is specified as a uniform read access over all data points, and a uniformly sampled subset of data points\techreport{\footnote{\blue{The insert queries in the training queries of the write-partial workload are sampled between 60\% and 90\% of the overall dataset.}}} to serve as key values for insert queries (with the exception of YCSB dataset). The ratio of read/insert queries is the same as in the target query workload.

\subsection{General Efficiency Comparison}\label{sec:general}
  In this section, we evaluate the performance of CARMI and compare against the baselines. We consider 5 different query workloads and 6 different datasets as explained in Section~\ref{sec:workload}. For synthetic and Open Street Map datasets, we consider 2 access patterns: uniform and Zipfian. These result in a total of 55 possible configurations. \techreport{Figure~\ref{fig:totalRes}} \paper{Figure~\ref{fig:totalResPaper}} shows the results for 35 of them due to space limitation, and the results for normal and exponential datasets are omitted since they are similar to those of the uniform dataset. 
  
  In general, the time efficiency of both learned indexes is significantly better than B+ Tree on all workloads. Comparing CARMI with ALEX, which is also a learned index, we see that these two learned indexes perform roughly the same over synthetic datasets. However, CARMI significantly outperforms over the OSMC dataset, achieving an average speedup of 1.45$\times$/3.78$\times$ on read-only/read-write workloads. This demonstrates the effectiveness of data partitioning and cache-aware design over real-world datasets, in which data location is much harder to predict.

\subsubsection{Read-only Workload}
  For read-only workloads, the lookup speed of CARMI is about 1.91-4.89$\times$ faster than B+ Tree under uniform access pattern, and 1.34$\times$ faster on average than ALEX, respectively. Meanwhile, CARMI uses only 0.64$\times$ of memory space compared to B+ Tree (excluding YCSB\footnote{For the YCSB dataset, since CARMI uses the external leaf nodes, which only store a pointer of the location of data points, the space cost of 11.4 MB only counts the space of the tree structure itself and does not include the space used by external data.} dataset).

  It is of interest to compare CARMI with B+ Tree, since their difference is only on the upper level. The significant speed gain of CARMI is mainly due to the following reasons: (a) CARMI uses fast model prediction instead of binary search. (b) the larger fanout of the root node in CARMI reduces the depth of the index. Because of these, most of the data points are managed by a leaf node that is directly under the root node, making the index structure flatter.

  Comparing the two learned indexes, the main difference is on the performance over OSMC, in which CARMI achieves a speedup of 1.47$\times$. The OSMC dataset is a real-world dataset with highly non-linear local distribution \paper{(the CDF can be found in our technical report~\cite{zhang2021carmi})}\techreport{(the CDF can be found in Figure~\ref{fig:cdf})}, which invalidates ALEX's strategy of storing data points according to the predicted location, and causes the index to grow deeper. Meanwhile, our hybrid construction algorithm can automatically select suitable nodes to make each subtree more balanced. Section~\ref{sec:sosd} shows similar results on other real-world datasets as well, making it clear that this is not a coincidence.

  In summary, CARMI outperforms B+ Tree and can achieve similar or better performance than ALEX under read-only workloads, and the gain is more evident on real-world datasets.

\paper{
  \begin{figure*}[ht]
    \centering
    % \setlength{\abovecaptionskip}{-3pt}
    \vspace{-0.6cm}
    \includegraphics[width=\linewidth]{./figure/cdf.pdf}
    \vspace{-0.6cm}
    \caption{The CDFs of Datasets in SOSD~\cite{marcus2020benchmarking}.}
    \Description{The CDFs of Datasets in SOSD~\cite{marcus2020benchmarking}.}
    \label{fig:cdf}
    \vspace{-0.3cm}
  \end{figure*}
}

  \techreport{
    \begin{table*}[ht]
     \center
     \caption{Results on SOSD Platform.}
     \label{tab:sosd}
     \begin{tabular}{c|cccccc|cccccccc}
       \toprule 
       ~&\multicolumn{6}{c|}{uint32}&\multicolumn{8}{c}{uint64}\\
      ~&uden&uspr&norm&logn&amzn &face&uden&uspr&norm&logn&amzn&face&wiki&osmc\\
      \midrule
      CARMI&158.43&170.62&176.43&180.82&192.84 &187.43 &165.43&186.43&169.42&177.87&201.80 & 334.41& 217.50&368.65 \\
      RMI&30.54 &143.23&75.43&102.43& 265.43&274.53&42.43&180.67&58.43&175.32 &266.54 &334.54  &222.43 &402.32  \\
      RS&35.98&190.73&73.66&85.08& 280.03 & 362.54&39.44&187.44&56.32&125.43 &296.61& 436.63 &218.43&412.39 \\
      ALEX&157.64&167.27&147.26&179.72&210.99  &434.69 &39.44&187.44&56.32&125.43 &251.32 & 496.48&  289.81&499.04 \\
      RBS&293.43&270.76&319.13&486.19& 325.43 &312.39 &167.61&185.46&159.32& 183.96 &385.96 &334.73 &335.75 &529.06   \\
      FAST&229.25&249.69&251.80&269.01& 246.03&228.79 &N/A&N/A&N/A &N/A &N/A&N/A&N/A &N/A  \\
      B+Tree&527.43&528.43&529.43&533.01& 529.43&524.54&599.32&602.43&604.23&598.32 &601.23&592.43 &608.42 &599.43 \\
      BS&965.20&974.21&970.19&915.01& 1014.5&983.49&1052.5&995.28&989.68&989.21 &1015.1&961.93 &1002.3&987.24 \\
      TIP&119.98&317.89&623.15&523.75& 731.97&880.12&192.43&376.43&685.27&286.74 &750.89&1124.6 &942.84 &4773.8 \\
      IS&30.00&324.78&8599.8&N/A& 3852.7&1007.7&35.21&352.29&9205.3&N/A &4103.9&1494.8 &6836.4&66474\\
     ART&104.31&N/A&179.72&N/A&N/A&182.36&112.27&264.23&226.03&302.43 &N/A&391.76&N/A&N/A  \\
      %  \midrule
      %  CARMI&146.32&168.43&155.43&177.43&167.43  &173.02&158.32&165.43&168.43& 172.54&205.32 & 352.34&  213.43&309.32\\
       \bottomrule
     \end{tabular}
   \end{table*}
   }
 

\paper{
  \subsubsection{Read-Write Workloads}
  For read-write workloads, CARMI achieves an average speedup of $2.14\times$/$2.13\times$ compared to B+ Tree and ALEX\footnote{The insert of the YCSB protocol is to continuously insert new data points at the end of the dataset, and ALEX does not strictly follow this mode for insert in their paper. Thus, our reported number is different compared to the values in their paper.}, while using 0.71$\times$/1.20$\times$ space on average.

  It is generally difficult for learned indexes to partition non-linear datasets evenly, leading to a large gap between the numbers of data points in each node. This results in additional expansion costs in ALEX during the insert operations. On the other hand, CARMI handles well even under such scenarios, using only 0.58$\times$ time of ALEX on lognormal/OSMC datasets.

  In summary, CARMI has a better time efficiency and uses a similar amount of space compared to ALEX, and the gap is more significant on non-linear and real-world datasets.
}

\techreport{
 \subsubsection{Write-heavy Workload}
  \purple{CARMI achieves an average speedup ratio of $2.24\times$ compared to B+ Tree and $1.88\times$ compared to ALEX\footnote{The insert of the YCSB protocol is to continuously insert new data points at the end of the dataset, and ALEX does not strictly follow this mode for insert in their paper. Thus, our reported number is different compared to the values in their paper.} on write-heavy workloads. Similar to the read-only case, CARMI demonstrates a strong performance on the uniform dataset compared with B+ Tree, having a speedup of  $3.56\times$.}
  
  \blue{It is generally difficult for learned indexes to partition non-linear datasets evenly, leading to a large gap between the numbers of data points in each node. This results in additional expansion costs in ALEX during the insert operations. On the other hand, CARMI handles well even under such scenarios, using only 0.49$\times$ time of ALEX on lognormal/OSMC datasets. As for space cost, CARMI uses 1.21$\times$ space compared to ALEX, and 0.72$\times$ compared to B+ Tree on average.}

  \blue{
    In summary, CARMI has a better time efficiency and uses a similar amount of space compared to ALEX, and the gap is more significant on non-linear and real-world datasets.}

 \subsubsection{Other Read-Write Workloads}
  \blue{CARMI has a shorter access time (2.10$\times$/2.21$\times$ average speedup comapred to B+ Tree and ALEX respectively) and use less space (0.77$\times$ on average compared to B+ Tree) for all other read-write workloads including range scan workload. This shows that CARMI can better handle various workloads, especially non-linear datasets.}

}

\subsection{SOSD Results}\label{sec:sosd} 
 In order to further test the performance of CARMI on real-world datasets, we have integrated CARMI into the SOSD benchmark~\cite{marcus2020benchmarking,sosd-vldb}, a platform for testing learned index structures. \paper{Table~\ref{tab:sosdPaper} shows the results of CARMI on the real-world datasets in the SOSD benchmark. The results on synthetic datasets can be found in the technical report~\cite{zhang2021carmi}.} \techreport{Table~\ref{tab:sosd} shows the results of CARMI on the datasets in the SOSD benchmark\footnote{\blue{In fact, a query requires at least one memory access (about 90ns), and the result reported by the SOSD benchmark is much less than this number. We suspect that in many test cases, the operating system predicts the location of the data to be accessed and prefetches it into the cache in advance. Due to this reason, the SOSD benchmark is overestimating the actual performance of some indexes (mostly simpler indexes that made such behavior possible).}}.} 
 
\paper{ 
  \begin{table}[ht]
   \center
   \caption{Results on SOSD Platform.}
   \vspace{-0.3cm}
   \label{tab:sosdPaper}
   \begin{tabular}{c|cc|cccc}
     \toprule 
     ~&\multicolumn{2}{c|}{uint32}&\multicolumn{4}{c}{uint64}\\
    ~&amzn &face &amzn&face&wiki&osmc\\
     \midrule
     CARMI&192.84 &187.43 &201.80 & 334.41& 217.50&368.65 \\
     RMI& 265.43&274.53 &266.54 &334.54  &222.43 &402.32  \\
     RS& 280.03 & 362.54 &296.61& 436.63 &218.43&412.39 \\
     ALEX&210.99  &434.69  &251.32 & 496.48&  289.81&499.04 \\
     RBS& 325.43 &312.39  &385.96 &334.73 &335.75 &529.06   \\
     FAST& 246.03&228.79   &N/A&N/A&N/A &N/A  \\
     B+Tree& 529.43&524.54 &601.23&592.43 &608.42 &599.43 \\
     BS& 1014.5&983.49 &1015.1&961.93 &1002.3&987.24 \\
     TIP& 731.97&880.12 &750.89&1124.6 &942.84 &4773.8 \\
     IS& 3852.7&1007.7 &4103.9&1494.8 &6836.4&66474\\
    ART&N/A&182.36 &N/A&391.76&N/A&N/A  \\
     \bottomrule
   \end{tabular}
 \end{table}
}
  
\paper{As shown in Table~\ref{tab:sosdPaper},}\techreport{As shown in Table~\ref{tab:sosd},} CARMI outperforms most of the baselines on the real-world datasets, which is consistent with our findings in Section~\ref{sec:general}. We also examine the distribution of datasets in SOSD benchmark, shown in Figure~\ref{fig:cdf}. As we can see, a major difference between synthetic and real-world datasets is that synthetic datasets all have locally linear CDF, which is generally not true for real-world datasets. \purple{The highly non-linear local CDFs of real-world datasets} make it nearly impossible to accurately predict the location of individual data records, which means that a large-range binary search is needed in the last mile. In contrast, since CARMI is designed based on the data partitioning perspective, and the leaf nodes use a fixed two-layer B-Tree structure, it can handle these highly non-linear parts better. The results on these real-world datasets reflect this difference, in which CARMI can achieve an average speedup of 1.21$\times$ compared to a well-tuned RMI. For completeness, we also report the average space usage of each index in Table~\ref{tab:sosdspace}.

\techreport{
\begin{table}[ht]
 \center
 \caption{Average Space Usage (MB) on SOSD.}
 \vspace{-5pt}
 \label{tab:sosdspace}
 \begin{tabular}{ccccccc}
   \toprule 
   ~&CARMI &RMI&RS&ALEX&RBS\\
   \midrule
   uint32 |& 3028.02 & 2475.92&2295.22 &3314.99 &2289.82 \\
   uint64 |& 4847.28& 3140.31&3060.12 &4414.38&3052.76 \\
   \midrule
   FAST&B+Tree&BS&TIP&IS&ART\\
   \midrule
  5120.00  &2657.31 &2288.82 & 2288.82&2288.82 &3776.20\\ 
  N/A &3540.52 &3051.76 &3051.76 &3051.76 &3821.61 \\
   \bottomrule
 \end{tabular}
\end{table}
}

\paper{
% \vspace{-0.3cm}
\begin{table}[ht]
 \center
 \caption{Average Space Usage (MB) on SOSD.}
 \vspace{-5pt}
 \label{tab:sosdspace}
 \begin{tabular}{ccccccc}
   \toprule 
   ~&CARMI &RMI&RS&ALEX&RBS\\
   \midrule
   uint32 |& 3918.30 & 2471.65&2299.63 &3336.74 &2289.82 \\
   uint64 |& 5481.44&3143.31&3064.33&4430.83&3052.76\\
   \midrule
   FAST&B+Tree&BS&TIP&IS&ART\\
   \midrule
  5120.00  &2657.31 &2288.82 & 2288.82&2288.82 &4596.52\\ 
  N/A &3540.52 &3051.76 &3051.76 &3051.76 &5280.92 \\
   \bottomrule
 \end{tabular}
\vspace{-0.2cm}
\end{table}
}

 In summary, the performance of existing learned indexes degrades heavily for locally non-linear datasets. CARMI on the other hand is more robust in such scenarios.
 

\subsection{Tradeoff between Time and Space}\label{sec:tradeoff}

One additional advantage of our cost-based index construction strategy is that one can now flexibly choose the balance point between time and space cost. As shown in Figure~\ref{fig:write-heavy}, by tuning the value of parameter $\lambda$ in Problem~\ref{prob:linear}, one can reduce the memory usage of indexes at the cost of increased read access latency. This suggests that in practice the database system can adjust the generated index's structure according to the hardware resources and time requirements to obtain a more desirable time/space tradeoff.

\begin{figure}[ht]
% \begin{figure}[t]
  \centering
  % \setlength{\abovecaptionskip}{-0.1cm}
  \includegraphics[width=8cm]{./figure/latency.pdf}
  \vspace{-0.3cm}
  \caption{The Trade-off Between Time and Space Cost}
  \Description{The trade-off between time and space}
  \label{fig:write-heavy}
  \vspace{-0.3cm}
\end{figure}

\techreport{  
  \begin{table*}[ht]
    \center
    \small
    \vspace{-0.3cm}
    \caption{Statistics on Different Root Fanouts.}
    \label{tab:ablationMemory}
    \vspace{-0.3cm}
    \begin{tabular}{c|ccc|ccc|ccc|ccc}
      \toprule  
\multirow{2}*{Root}&\multicolumn{3}{c|}{Uniform Dataset}&\multicolumn{3}{c|}{Normal Dataset}&\multicolumn{3}{c|}{Lognormal Dataset}&\multicolumn{3}{c}{OSMC Dataset}\\
~&\multirow{1}*{Time}&\# of&\multirow{2}*{Percentage}&\multirow{1}*{Time}&\# of&\multirow{2}*{Percentage}&\multirow{1}*{Time}&\# of&\multirow{2}*{Percentage}&\multirow{1}*{Time}&\# of&\multirow{2}*{Percentage} \\
Fanout&/ns&Accesses&~&/ns&Accesses&~&/ns&Accesses&~&/ns&Accesses&~ \\
      \midrule
      65536  &301.64&6.82&5.14\%&355.39&7.67&4.76\%&372.72&8.73&3.32\%&593.10&11.95&0.22\%\\ 
      131072 &280.58&5.72&7.28\%&333.46&6.66&6.74\%&337.73&7.69&4.68\%&539.83&11.15&0.38\%\\ 
      262144 &254.16&4.62&10.36\%&300.26&5.65&9.58\%&308.69&6.64&6.62\%&487.83&10.33&0.67\%\\ 
      524288 &212.34&3.52&14.66\%&276.09&4.65&13.55\%&283.86&5.58&9.35\%&449.08&9.52&1.14\%\\ 
      1048576&168.43&2.47&20.66\%&232.51&3.68&19.05\%&261.56&4.54&13.05\%&410.11&8.69&1.89\%\\
      2097152&152.71&1.53&28.64\%&212.36&2.80&26.25\%&230.68&3.53&17.99\%&374.43&7.85&3.05\%\\
      \bottomrule
    \end{tabular}
  \end{table*}
}

\subsection{Cost of Construction}\label{sec:cost}

The construction of the index structure should only be performed periodically when the database system has enough computation resources to spare (e.g., during night time when the frequency of the incoming queries is low). As such, the time efficiency of the construction algorithm is not a major concern. Nevertheless, we still want to have a basic understanding of its time cost.

Recall that we have two algorithms (the greedy algorithm and the DP algorithm) to construct a node. In order to achieve a balance between the construction time and efficiency, we define a parameter $kAlgorithmThreshold$ in CARMI, and use the greedy algorithm when the size of the sub-dataset is greater than the parameter. Figure~\ref{fig:time} shows the time required by the algorithm at different parameter values for all datasets. As we can see, the construction of indexes can be finished within 1-4 minutes for a 1GB dataset, which is generally acceptable for most practical scenarios. Note that the longlat dataset is a combination of actual latitude and longitude data and is highly non-linear. Therefore, the construction time of this dataset is longer than the other datasets.

\begin{figure}[ht]
% \begin{figure}[t]
  \centering
  \includegraphics[width=8cm]{./figure/time.pdf}
  \vspace{-0.3cm}
  \caption{Running Time of Construction Algorithm}
  \Description{Running time of construction algorithm}
  \label{fig:time}
  \vspace{-0.3cm}
\end{figure}

It is worth noting that if we do not use the greedy algorithm, the construction time will be much longer. Therefore, we take full advantage of the different strengths of the two algorithms and use them to reduce the construction time of CARMI.

% \subsection{Multi-Platform Comparison} \label{sec:platform}
% Since different operating systems and hardware all have their own memory prefetching mechanism, they can potentially interfere with the normal operation of CARMI. To characterize the effect of such difference, we conducted additional read-only experiments on two other platforms: (1) a Windows machine equipped with an Intel Core i9-10900K CPU (3.70 GHz). (2) a macOS machine with an Intel Core i5 and 16GB RAM. Figure~\ref{fig:platform} shows the results.

% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=8cm]{./figure/platform.pdf}
%   % \vspace{-5pt}
%   \setlength{\abovecaptionskip}{-0.03cm}
%   \caption{Time on Different Platforms}
%   \Description{Time on Different Platforms}
%   \label{fig:platform}
% 	\vspace{-5pt}
% \end{figure}

% As we can see, due to the difference in memory latency of each platform, the average time usage of each index also shows slight variation across the platforms. However, the more interesting phenomenon is that the ratio between the longest and shortest time for each index among the three platforms also varies greatly: \purple{2.55$\times$ for CARMI, 3.57$\times$ for ALEX \orange{ and 1.54$\times$ for B+ Tree}. For ALEX,} the gap between them on different platforms is most likely due to the fact that the prefetching mechanisms of Ubuntu and Windows platforms are more suitable for this experiment, which results in better results compared to macOS platform. As for CARMI, the cache-aware design and the built-in prefetching mechanism make it less dependent on the hardware/OS level prefetching, resulting in a smaller difference than ALEX. \orange{To conclude, CARMI's special design makes it very robust on different platforms.}

\techreport{
%   \begin{table*}[ht]
%     \center
%     \vspace{-0.3cm}
%     \caption{Statistics on Different Root Fanouts.}
%     \label{tab:ablationMemory}
%     \vspace{-0.3cm}
%     \begin{tabular}{c|ccc|ccc|ccc}
%       \toprule  
% \multirow{2}*{Root Fanout}   &\multicolumn{3}{c|}{Uniform Dataset}&\multicolumn{3}{c|}{Normal Dataset}&\multicolumn{3}{c}{Lognormal Dataset}\\
%    &Time/ns&Search Range&Percentage&Time/ns&Search Range&Percentage&Time/ns&Search Range&Percentage \\
%       \midrule
%       65536& 295.6&565.9& 5.14\% &345.8&86586.6&4.76\%&363.4&24927.2& 3.32\% \\ 
%       131072&275.3&273.7&7.28\%&319.3&86294.4&6.74\% &332.8&23741.9&4.68\% \\ 
%       262144&232.8&130.3&10.36\%&287.4&86151.1&9.58\% &298.8&23155.1&  6.62\% \\ 
%       524288& 177.5&60.9&14.66\%&243.2&86081.4&13.55\%&273.1&22865.3&  9.35\%\\ 
%       1048576 &162.1&28.1 &20.66\%&228.2&86047.9&19.05\%&249.7&22723.3 &13.05\%\\
%       2097152 &153.8&12.9 &28.64\%&218.5&86032.3 &26.25\%&210.2&22654.5 &17.99\% \\
%       \bottomrule
%     \end{tabular}
%   \end{table*}
  % \begin{table*}[ht]
  %   \center
  %   \vspace{-0.3cm}
  %   \caption{Statistics on Different Root Fanouts.}
  %   \label{tab:ablationMemory}
  %   \vspace{-0.3cm}
  %   \begin{tabular}{c|c|cccccc}
  %     \toprule  
  %     \multicolumn{2}{c|}{Root Fanout}&65536&131072&262144&524288&1048576&2097152\\
  %     \midrule
  %     \multirow{3}*{Uniform Dataset}&Time/ns&301.64&280.58&254.16&212.34&168.43&152.71\\
  %     ~&Avg Number of Memory Accesses&6.82&5.72&4.62&3.52&2.47&1.53\\
  %     ~&Avg Number of Data Points&&&&&\\
  %     \midrule
  %     \multirow{3}*{Normal Dataset}&Time/ns&355.39&333.46&300.26&276.09&232.51&212.36\\
  %     ~&Avg Number of Memory Accesses&7.67&6.66&5.65&4.65&3.68&2.80\\
  %     ~&Avg Number of Data Points&&&&&\\
  %     \midrule
  %     \multirow{3}*{Lognormal Dataset}&Time/ns&372.72&337.73&308.69&283.86&261.56&230.68\\
  %     ~&Avg Number of Memory Accesses&8.73&7.69&6.64&5.58&4.54&3.53\\
  %     ~&Avg Number of Data Points&&&&&\\
  %     \midrule
  %     \multirow{3}*{OSMC Dataset}&Time/ns&593.10&539.83&487.83&449.08&410.11&374.43\\
  %     ~&Avg Number of Memory Accesses&11.95&11.15&10.33&9.52&8.69&7.85\\
  %     ~&Avg Number of Data Points&&&&&\\
  %     \bottomrule
  %   \end{tabular}
  % \end{table*}
  \subsection{The Effect of Fanout}\label{sec:fanout}
  \purple{In order to show the effect of root fanout on average access time, we use CARMI to simulate a two-layer static RMI with adjustable root fanout. The root node, which is the linear regression model, directly manages the leaf nodes. Each leaf node is the external array leaf node. Table~\ref{tab:ablationMemory} shows the average access time under different root fanouts and the average number of memory accesses required in the process. We also count the percentage of data points that are stored in the same location as the location calculated by the linear model across all data points.}

  \purple{The statistics in Table~\ref{tab:ablationMemory} demonstrate that the average time tends to be smaller as the fanout increases. The results show several conclusions: (a) Reducing the number of memory accesses can effectively reduce the average access time. The 5.29 fewer memory accesses for the uniform dataset saves an average access time of 148.93 ns. Therefore, we suggest that learned indexes need to be designed based on the main memory, such as our cache-aware design. It should be noted here that the actual time is less than the theoretically required time. This is due to the built-in software and hardware optimizations such as prefetching instructions, instruction reordering, etc., which can speed up binary search in some cases. (b) The larger the fanout, the larger the proportion of correct predictions. It means that the appropriate increase of fanout can simplify the situation of lower-level nodes, so that leaf nodes can process queries faster, which proves the necessity of simplifying the situation of lower-level nodes mentioned in Section~\ref{sec:preliminary}. (c) For the OSMC dataset, even with a fanout of 2,097,152, it cannot handle such a real-world dataset well and still requires an average of more than seven memory accesses, indicating the need for the CARMI framework.}

  \purple{In summary, fanout significantly impact the performance of the index. Therefore, the index needs to be designed around the aspect, which is reflected in the entropy metric of CARMI.  Moreover, our cache-aware design and prefetch mechanism are to minimize the number of memory accesses.}
  \subsection{Ablation Experiments}\label{sec:ablation} 

  \subsubsection{Model Characteristics} 
  \purple{Next, we investigate the impact of our design on the overall performance. First, we conduct experiments on the four inner nodes in Appendix~\ref{sec:innerdetails} to show their respective characteristics. The root nodes are all consistent piecewise linear nodes in Appendix~\ref{sec:plrroot}, and other parameters are the same, but only one kind of node can be used as inner nodes.} %Here the $\lambda$ parameter is different from it in Section~\ref{sec:general}, so the results are different.

  \purple{Table~\ref{tab:ablationModel} shows that these inner nodes have their own merits. For the uniform dataset, the LR model can evenly distribute the data points to the lower nodes with the shortest computation time, showing better performance than other models. However, it always concentrates many data points into a few child nodes for non-linear datasets and the shortest calculation time cannot compensate for the disadvantages of low entropy. The P. LR model aims to maximize the entropy, so it beats other models and only needs 152.5 ns on the normal dataset. As for the lognormal and OSMC dataset, the models other than the BS model are sensitive to the data distribution, which means that they cannot obtain good benefits in extreme cases. Therefore, BS models can perform better due to the strongest ability to divide data.}

  \begin{table}[ht]
    \center
    \vspace{-0.2cm}
    \caption{Latency on Different Model Types.}
    \label{tab:ablationModel}
    \vspace{-0.3cm}
    \begin{tabular}{c|cccc|c}
      \toprule  
     ~&LR  &P. LR  &His  &BS  &CARMI\\
      \midrule
      Uniform& 136.8& 143.5& 141.3&145.8&136.6\\ 
      Normal&153.6&152.5&158.7&154.9&139.4\\ 
      Lognormal&157.5&155.0&155.8&153.8& 139.9\\
      OSMC&415.8 &405.3 &413.32 &374.9 & 293.4\\
      \bottomrule
    \end{tabular}
  \end{table}

  \purple{In summary, each model can have its own suitable scene, and it makes sense to combine them together. Based on our fixed-size node design, this can be easily achieved. The results of CARMI are also shown in Table~\ref{tab:ablationModel}. Benefiting from our hybrid construction algorithm and cost model, CARMI chooses the optimal node settings under different situations to get the shortest average access time.}

  \subsubsection{Prefetching Mechanism} 
  \purple{In order to evaluate the impact of the prefetching mechanism, we conduct ablation experiments with and without prefetching instructions on these four datasets and show the time/space costs and the proportion of data blocks that are successfully prefetched in Table~\ref{tab:prefetch}. On these synthetic datasets, the average success rate of the prefetching mechanism is 93.1\%, and the average access time is reduced by 63.1 ns. For real-world datasets, most data points require at least two inner nodes to handle the data distribution, so there is little gain in prefetching them at the root node. As we discussed in Section~\ref{sec:prefetch}, the prefetching mechanism requires more space to better exert its effects.}

  \begin{table}[ht]
    \center
    \small
    \vspace{-0.2cm}
    \caption{Results With/Without Prefetch Mechanism.}
    \label{tab:prefetch}
    \vspace{-0.3cm}
    \begin{tabular}{c|ccc|cc}
      \toprule  
     ~&\multicolumn{3}{c|}{with prefetch}&\multicolumn{2}{c}{without prefetch}\\
     ~&time& space&proportion &time& space\\
      \midrule
      Uniform&114.0& 1509.3&98.3\%& 185.8&1230.6\\ 
      Normal&124.6&1561.6&89.1\%&184.4&1334.2 \\ 
      Lognormal&126.2&2137.8&91.9\%&183.7&1912.4 \\
      OSMC&284.5&1557.86&2.5\%&289.3&1533.4\\
      \bottomrule
    \end{tabular}
  \end{table}
 }

\techreport{
\subsection{Tree Structure}\label{sec:tree}
 \blue{To understand the behavior of the index construction algorithm, we have gathered statistics on the optimal indexes constructed by the algorithm, and some of them are shown in Table~\ref{tab:statistic}. We follow the convention that the depth of a trivial tree (with only root node) is 1, and count depth on the leaf node level. The average is calculated with respect to keys.}

\blue{The first two columns are statistics under a read-only workload. As we can see, the algorithm constructs an average two-layer structure for uniform dataset under read-only workloads: the first layer is the LR root node and the second layer are the CF array leaf nodes. When performing a read query, we only need to access a single leaf node and a single data block. Due to the distributional variation caused by the sampling process, a small number of data points need an additional inner node.}
\begin{table}[ht]
	\center
  \small
	\caption{Statistics of Indexes Constructed by CARMI.}
	\label{tab:statistic}
	\begin{tabular}{c|cc|cc}
    \toprule
    ~&\multicolumn{2}{c|}{read-only}&\multicolumn{2}{c}{lognormal}\\
    node&uniform &normal&write-heavy&write-partial\\
    \midrule
    root node   & LR & P. LR&P. LR &P. LR \\
    \# of children   &1175653 & 1175653& 1528348&1528348\\
    \midrule
  \# of LR&2& 835&4690&4697\\
  \# of P. LR& 0&4&8&8\\
  \# of His& 0&2&2&0\\
  \# of BS&0 &0&0&1\\
    \midrule
    Array& 1175685&1320524&1784066&1767682\\
    \midrule
    Max Depth&3&3&4&4\\
    Avg Depth&2&2.03&2.07&2.07\\
		\bottomrule
	\end{tabular}
\end{table}

\blue{For other datasets, we can no longer construct a simple two-layer index to handle the dataset as the data points are very concentrated in a specific range, which cannot be handled by a single leaf node. As we can see, the root node setting changes depending on the data distribution and CARMI chooses to use P. LR for all the other three scenarios. We also see that the algorithm generates new inner nodes to partition the data points further, and builds deeper subtrees in more concentrated parts of the data points. Aside from the deep part, the algorithm maintains a shallow free structure in the other parts to guarantee that the average depth is small, achieving an average depth of 2.03-2.07.}

\blue{As we can see in Table~\ref{tab:statistic}, depending on the data distribution, the algorithm will adaptively use the four types of inner nodes. For example, in lognormal dataset under write-partial workload, CARMI constructed $4697$ LR nodes in the evenly distributed part, and $8$ P. LR nodes in the unevenly distributed part. In general, CARMI can effectively handle different data distributions and diverse workloads, and construct a reasonable index structure accordingly. These results also justify the decision of including multiple tree node types in CARMI, which enhances the flexibility of index structures.}
} 

==> tex/introduction.tex <==
\setcounter{page}{1}
\section{Introduction}
Index structure, as an indispensable access method in database systems, is of great significance to support efficient data access. Most traditional indexes are general-purpose, in the sense that they store data based on a single fixed rule and do not take advantage of the characteristics of data distribution. One would hope that machine learning (ML) techniques can be integrated into index structures to allow them to take advantage of data distribution regularity and improve their efficiency and flexibility.

This new direction was first explored by Kraska et al.~\cite{kraska2018case}, in which they used ML techniques to build database indexes. They proposed a data structure called Recursive Model Index (RMI) to connect many ML model nodes together in a hierarchical manner. Given a key value, one traverses through the index structure using ML models to determine the next branch, and finally arrives at a position in the data array and performs the last mile search within the error range. Kraska et al.~\cite{kraska2018case} used a proof-of-concept design to demonstrate the idea that ML models as indexes (a.k.a. learned indexes) can potentially provide faster search time compared to a traditional B+ Tree.

\revision{According to the SOSD benchmark~\cite{marcus2020benchmarking}, which evaluates the performance of learned indexes, there is a gap in the performance of RMIs between real-world and synthetic datasets, and the average access time required on the former is 2.92$\times$ of the latter. Most current RMIs~\cite{ding2019alex, radixspline, stoian2021plex, galakatos2018tree,marcus2020cdfshop, ferragina2020pgm,kraska2018case} do not address this issue and have performance degradation in real applications~\cite{marcus2020benchmarking}.}

\revision{In this paper, we explain this gap from three aspects and propose three novel ideas to address each of them:}

\revision{\textbf{\textit{1) Model Fitting View.}} The core idea of the current RMIs is the model fitting view, where the goal of each ML model is to accurately fit the cumulative distribution function (CDF) of the corresponding sub-dataset so that input keys can be precisely mapped to their locations. This view means that ML models in leaf nodes are fitting local distributions of the dataset.}

\revision{The model fitting view leads to a performance gap of RMIs on real-world datasets and synthetic datasets due to a significant difference between them. More specifically, local data distributions of synthetic datasets are linear, while real-world datasets are not. Because of this, the models in leaf nodes can always fit the local CDFs of synthetic datasets well, which is not the case in real-world datasets.}

\revision{To deal with this issue, we propose to design RMI frameworks from a data partitioning view. In this view, instead of accurately fitting CDFs, upper-level models should focus on dividing datasets into small chunks, which can simplify the situation in lower levels and reduce the tree height for a flatter structure. Then, the lower-level nodes can easily process these small sub-datasets, avoiding performance degradation.}

\revision{In the data partitioning view, the utility of individual tree nodes is reflected in the effectiveness of data partitioning. As long as the data partitioning effectiveness is the same, complex models that sacrifice computation time for better fitting can be replaced by simple models, which can also reduce the average time. We propose to use entropy, an information-theoretic metric~\cite{gray2011entropy}, to quantify the data partitioning effectiveness and derive a formula to characterize the performance of each node with local information.}

\revision{\textbf{\textit{2) Inflexible Index Construction.}} Automatically tuning tree structures and model types of RMIs can effectively shorten the performance gap of manually tuned RMIs and obtain flexible and better index structures~\cite{marcus2020cdfshop, sosd-vldb}. More specifically, manually tuned RMIs have a performance gap on real-world and synthetic datasets since the simpler data distributions of synthetic datasets make it easier to adjust RMIs manually. There are some existing works~\cite{ding2019alex,wu2021updatable,marcus2020cdfshop} attempting to construct indexes automatically, but they all have shortcomings. Some of them~\cite{ding2019alex,wu2021updatable} only use linear models for simplicity, requiring model types in tree structures to be fixed. CDFShop~\cite{marcus2020cdfshop} determines node types in each layer of the original RMI ahead of time and then uses program synthesis techniques to create an actual implementation, which requires recompilation. In short, these existing works cannot automatically tune both model types and tree structures at runtime.}

\revision{In this paper, we aim to design an index framework that can automatically tune the above aspects. To this end, we formalize the index construction problem as an optimization problem using a cost model that will be described in Section~\ref{sec:framework} and design a hybrid algorithm to solve it. This algorithm can flexibly construct indexes with good performance at runtime without the need for manual tuning and recompilation. Furthermore, we also propose a novel dynamic architecture based on the memory layout described below. This architecture supports variable tree depths and allows each tree node to have different types and numbers of children, further enhancing the flexibility of index structures.}

\revision{\textbf{\textit{3) Performance Bottleneck of Memory Access.}} Memory access time dominates the average lookup time in RMIs~\cite{sosd-vldb}, and thus, we should strive to avoid extra cache misses compared to existing RMIs when designing a new index framework. We first exploit the behavior characteristics of CPU cache memory to propose a novel cache-aware design with a new memory layout. Since the size of data fetched by a single memory access is fixed, our design requires that all tree nodes have a fixed size equal to the cache line size (64 bytes) and are stored in a single array to align the cache line. Then, we can make full use of these 64 bytes to design various nodes to handle different situations for better index structures. With such a design, we neither need additional memory access to fetch nodes nor waste data fetched into the cache.}

\revision{Memory access is not only the performance bottleneck of RMIs, but also a reason for the performance gap of RMIs on real-world and synthetic datasets. More specifically, since ML models cannot fit real-world datasets well as we mentioned earlier, the model error, which is the difference between predicted position and actual position, becomes larger than that on synthetic datasets, resulting in much larger error-based search ranges in the last mile~\cite{marcus2020cdfshop, ding2019alex,radixspline,kraska2018case}. These large-range searches across multiple memory blocks incur more memory accesses, leading to the performance gap.}

\revision{To address this issue, we design a new leaf node with a similar concept of a two-level B+ Tree node, consisting of a 64-byte root and multiple 256-byte data blocks. This leaf node only uses one memory access to narrow down the search range to 256 bytes with the 64-byte metadata, and then performs searches within this 256-byte block. Compared to large-range searches in some RMIs~\cite{marcus2020cdfshop, ding2019alex,radixspline,kraska2018case} that require more memory accesses to narrow search ranges, this leaf node can effectively reduce the number of memory accesses on real-world datasets, thereby shortening the performance gap.}

\revision{In conclusion, we integrate all the above new ideas and propose a novel cache-aware RMI framework, called CARMI, to improve the performance of RMIs, especially on real-world datasets.}

The contributions of this paper are listed as follows:
\begin{itemize}[leftmargin=*]
\vspace{-3pt}
\item \revision{We propose a new data partitioning view for the RMI framework and introduce a new metric, called entropy, which makes it possible to analyze and quantify the performance of tree nodes in a standalone fashion.}
\item \revision{To support flexible index construction, we formalize the index construction problem as an optimization problem, and propose a dynamic architecture and a hybrid algorithm for solving it.}
\item We propose CARMI, a novel RMI framework equipped with a new memory layout that better utilizes the cache to effectively reduce the ``last mile'' search time and improve the overall performance. In addition, we utilize memory prefetch instructions to parallelize memory access and further reduce access latency.
\item \revision{CARMI is a generic framework that allows users to design new nodes and} we provide an implementation of CARMI~\cite{carmiGithub} with six example designs of tree nodes as references.
\item We conduct a series of experiments to demonstrate the strong performance and robustness of our framework.
\end{itemize}

The remainder of this paper is outlined as follows: In Section~\ref{sec:preliminary}, we review the RMI framework and discuss the two ways of viewing RMI: model fitting vs. data partitioning. In Section~\ref{sec:framework}, we derive a cost model for the entire index structure, and introduce entropy as a metric for characterizing the node performance. Section~\ref{sec:constructionAlg} discusses the cost-based hybrid index construction algorithm, which is used to choose different node settings flexibly to construct the optimal index structure during runtime. In Section~\ref{sec:cache}, we explain the cache-aware designs of CARMI, including the new memory layout and a prefetching mechanism. The experimental setup and results are shown in Section~\ref{sec:experiment}. We discuss the possible extension directions and future works in Section~\ref{sec:discussion}. Finally, we discuss related work in Section~\ref{sec:related} and conclude in Section~\ref{sec:conclusion}. \techreport{Some implementation details, experimental settings and proof of theorem can be found in the appendix.}


==> tex/preliminary.tex <==
\section{RMI and Partition View}\label{sec:preliminary}
\subsection{Two Different Views}
Figure~\ref{fig:learnedIndex} shows the index structure of Recursive Model Index (RMI), which is a ML-based index framework. Each inner node in the RMI represents an order-preserving regression model: the model $f: k \rightarrow idx$ takes key value $k$ as input, and outputs an integer $idx \in \{1, 2, \ldots, c\}$, where $c$ is the number of child nodes of this inner node. The order-preserving property is defined as $k_1 \leq k_2 \Rightarrow f(k_1) \leq f(k_2)$, which ensures that RMI can handle range queries properly. Leaf nodes in the bottom layer use linear models to manage data points. Then, using RMI to find data points matching input key value $k$ is straight-forward: starting from the root, we repeatedly call the model to determine which branch we will visit for the next iteration until we reach a leaf node. Finally, a binary search is performed in it to retrieve the matching records.
\begin{figure}[ht]
  \centering
  \vspace{-0.3cm}
  \includegraphics[width=\linewidth]{./figure/learnedIndex.pdf}
  \vspace{-0.5cm}
  \caption{Learned Index}
  \Description{Learned Index}
  \label{fig:learnedIndex}
  \vspace{-0.3cm}
\end{figure}

In the original RMI paper~\cite{kraska2018case} and the follow-up ones~\cite{marcus2020cdfshop, ding2019alex, radixspline, stoian2021plex, galakatos2018tree, ferragina2020pgm}, the behavior of RMI is viewed from the perspective of model fitting. In this view, each model is trained to minimize a loss function (e.g., squared loss funtion) and fit the CDF of a given dataset. Then, a good model is one that minimizes the loss function well on a given sub-dataset. More specifically, models of root nodes aim to fit CDFs of entire datasets and models of leaf nodes fit their local distributions.

Model fitting view leads to a performance gap of RMIs~\cite{marcus2020benchmarking} between synthetic and real-world datasets due to their different local distributions. Because of the locally linear distributions of synthetic datasets, ML models of leaf nodes can fit them well and predict positions close to actual positions. Thus, only small-range searches surrounding predicted positions are required to accurately locate data points. In contrast, the local distributions of real-world datasets are highly non-linear\footnote{The CDFs of synthetic and real-world datasets are shown in Section~\ref{sec:sosd}.}, which makes it hard for models to fit them well and predicted positions are far from actual positions. Then, additional procedures (e.g., large-range searches) are required to locate data points accurately. These large-range searches span many memory blocks and require multiple memory accesses, resulting in performance degradation in practical scenarios.

To shorten the performance gap, we propose to use a data partitioning view to design the RMI framework, where each model aims to partition a given dataset more evenly into smaller chunks. In this view, rather than the loss of each model, we are more concerned with the effectiveness of data partitioning, that is, the ability of tree nodes to partition datasets. Then, upper-level models can have a larger fanout to divide datasets into smaller sub-datasets to obtain better data partitioning effectiveness.

Our proposed view can effectively reduce the performance gap of RMIs between different datasets. First, lower-layer nodes can more easily handle simplified situations since they can get smaller sub-datasets from upper-layer nodes. Then last-mile search ranges can be effectively shortened, thus reducing the number of memory accesses on real-world datasets. Second, we can form flatter index trees on non-linear datasets instead of uneven and skewed trees, thereby reducing cache misses caused by deeper trees.

In this paper, we propose to use entropy, an information-theoretic metric~\cite{gray2011entropy}, to formally quantify the data partitioning effectiveness. Suppose an inner node $M$ distributes a total of $n$ data points into $c$ different child nodes\footnote{Note that the number of child nodes of an inner node is also part of the model configurations and we need to determine its optimal value when constructing the index.}, then the entropy $H(M)$ is defined as: $H(M) = -\sum_{i=1}^{c} p_i \log_2 p_i$, where $p_i = \frac{n_i}{n}$ and $n_i$ is the number of data points allocated to the $i$-th child node. Larger entropy means that datasets are divided more evenly into smaller ones, which is preferable since it leads to a more balanced tree. Moreover, entropy can also aid in establishing the notion of local node efficiency in Section~\ref{sec:theoreticalAnalysis}, which combines time/space cost of a single node and its dataset partitioning utility into a single metric. With this metric, we can effectively compare models locally without global information, thus speeding up index construction.

\subsection{Overview of CARMI}\label{sec:overview}
In this paper, we extend the RMI framework and propose a refined general RMI framework that can automatically build suitable and updatable indexes for given datasets, called Cache-Aware RMI (CARMI). CARMI retains RMI's core idea of replacing traditional indexes with ML models and has similar procedures for querying data points, but differs in specific designs. Specifically, in our new memory layout (\cref{sec:cache}), all tree nodes are limited to 64 bytes and stored in a single array. Then, according to the independent characterization of each tree node (\cref{sec:framework}), CARMI can use different nodes to handle different sub-datasets and link them into an index tree.

Nodes in CARMI are explicitly classified into two categories: inner nodes and leaf nodes. Inner nodes are intermediate bridges between root and leaf nodes, using models to determine the next branch. Leaf nodes are similar in concept to leaf nodes of B+ Tree, but they only store data points conceptually by storing pointers to data blocks containing actual data points.

For a given dataset, CARMI uses a hybrid construction algorithm (\cref{sec:constructionAlg}) to solve the index construction problem, whose optimization objective is to minimize the weighted sum of time and space costs (\cref{sec:framework}). With this algorithm, CARMI can automatically construct indexes with good performance at runtime.

Then, we illustrate the design of CARMI via a concrete example:
\begin{figure}[ht]
  \vspace{-0.4cm}
  \centering
  \includegraphics[width=\linewidth]{./figure/example.pdf}
  \vspace{-0.6cm}
  \caption{A Simple Example of CARMI}
  \Description{Example}
  \label{fig:example}
\vspace{-0.6cm}
\end{figure}
\begin{example}\label{example1}
Consider a dataset in which there are 500 data points $D = \{0, 1, \cdots 199, 200, 202, \cdots, 798\}$. Then CARMI can be a four-layer structure, as shown in Figure~\ref{fig:example}. The top layer is the root node with a linear regression (LR) model ($idx = \lfloor 0.005 \times key \rfloor$), which determines the index of the next node for each given key. The first 200 data points are managed by an LR inner node and its two child leaf nodes. The remaining 300 data points are directly managed by 3 leaf nodes ($M_1-M_3$). Each leaf node is linked to 7 data blocks at the bottom and uses them to store data points.

Suppose that we need to access the record with key value $592$. We first access the root node and use its model to calculate the index of the next node ($idx = \lfloor 0.005 \times 592 \rfloor = 2$). After obtaining the content of $M_2$, we use its strategy to get the index of the data block ($L_{27}$), and finally, search for the key value $592$ within $L_{27}$. Since the root node is frequently accessed, we assume that it is always in the cache memory. Therefore, for this example, we only need two random memory accesses: the leaf node $M_2$ and the data block $L_{27}$, respectively.
\end{example}

